Empirical Results for Adjusting Truncated Backpropagation Through Time while Training Neural Audio Effects

This paper investigates the optimization of Truncated Backpropagation Through Time (TBPTT) for training neural networks in digital audio effect modeling, with a focus on dynamic range compression. The study evaluates key TBPTT hyperparameters -- sequence number, batch size, and sequence length -- and their influence on model performance. Using a convolutional-recurrent architecture, we conduct extensive experiments across datasets with and without conditionning by user controls. Results demonstrate that carefully tuning these parameters enhances model accuracy and training stability, while also reducing computational demands. Objective evaluations confirm improved performance with optimized settings, while subjective listening tests indicate that the revised TBPTT configuration maintains high perceptual quality.

==> table_lc_median.tex <==
\begin{table*}[htb]
\centering
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabularx}{\linewidth}{{llXXXXXXXXX}}
\toprule
 & $L_c$ & 4096 & 8192 & 12288 & 16384 & 24576 & 32768 & 49152 & 65536 & 98304 \\
$B$ & $N$ &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{3}{*}{8} & 1 & {\cellcolor[HTML]{EB5A3A}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FA9B58}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FAFDC9}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{78B0D3}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{A90426}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FEE99D}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{81B7D7}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4471B2}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{F46D43}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{A3D3E6}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4D7FB9}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{16} & 1 & {\cellcolor[HTML]{F57245}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FFF6B1}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{9DCEE3}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{35429B}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{FDAF62}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FEEFA6}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{4D7FB9}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{FED889}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{DAF0F6}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{5183BB}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{3A51A2}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{32} & 1 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FDBB6D}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{588CC0}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{3E60AA}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{FEE99D}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{F0F9DB}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{78B0D3}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{CFEBF3}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4B7DB8}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{4D7FB9}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{64} & 1 & {\cellcolor[HTML]{FCA85E}} \color[HTML]{000000}  & {\cellcolor[HTML]{FEEBA1}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{5C90C2}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{416AAF}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{FECE7F}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{D1ECF4}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4878B6}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{333D99}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{FDC778}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{C7E7F1}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4878B6}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{384CA0}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{128} & 1 & {\cellcolor[HTML]{FEE294}} \color[HTML]{000000}  & {\cellcolor[HTML]{FFF8B5}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{8EC2DC}} \color[HTML]{000000}  &   &   &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{5E93C3}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 3 &   &   & {\cellcolor[HTML]{FEECA2}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{E2F4F4}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4878B6}} \color[HTML]{F1F1F1}  &   &   \\
\bottomrule
\end{tabularx}
\caption{snapshot}
\label{tab:lc_median_snap}
\end{subtable}
\hfill
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabularx}{\linewidth}{{llXXXXXXXXX}}
\toprule
 & $L_c$ & 4096 & 8192 & 12288 & 16384 & 24576 & 32768 & 49152 & 65536 & 98304 \\
$B$ & $N$ &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{3}{*}{8} & 1 & {\cellcolor[HTML]{A90426}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{E44C34}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{F99355}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FED889}} \color[HTML]{000000}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{DB382B}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{F7844E}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FECC7E}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FFF3AD}} \color[HTML]{000000}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{F26841}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FECA7C}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FEE699}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{DAF0F6}} \color[HTML]{000000}  \\
\multirow[c]{3}{*}{16} & 1 & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{F26841}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FDB164}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{E9F6E8}} \color[HTML]{000000}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FCA85E}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FBFDC7}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{9FD0E4}} \color[HTML]{000000}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{FCA55D}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FED485}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FCFEC5}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{32} & 1 & {\cellcolor[HTML]{C41E27}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{F36B42}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{EDF8DF}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{4065AC}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{F47044}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FDB567}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{D4EDF4}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{6399C7}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{F8864F}} \color[HTML]{F1F1F1}  &   & {\cellcolor[HTML]{FEC87A}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{DAF0F6}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{74ADD1}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{64} & 1 & {\cellcolor[HTML]{CE2827}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FDC374}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FEECA2}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{3E60AA}} \color[HTML]{F1F1F1}  &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{F99355}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FDBB6D}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{81B7D7}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{679EC9}} \color[HTML]{F1F1F1}  &   \\
 & 3 &   &   & {\cellcolor[HTML]{FA9857}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{FED283}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{92C5DE}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1}  \\
\multirow[c]{3}{*}{128} & 1 & {\cellcolor[HTML]{C62027}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FEE699}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{87BDD9}} \color[HTML]{000000}  &   &   &   &   &   \\
 & 2 &   & {\cellcolor[HTML]{FA9656}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{EAF7E6}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{85BBD9}} \color[HTML]{000000}  &   &   &   \\
 & 3 &   &   & {\cellcolor[HTML]{FBA35C}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{CFEBF3}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{7AB2D4}} \color[HTML]{000000}  &   & {\cellcolor[HTML]{6399C7}} \color[HTML]{F1F1F1}  \\
\bottomrule
\end{tabularx}
\caption{Threshold-Ratio}
\label{tab:lc_median_threshratio}
\end{subtable}
\hfill
\caption{Median values of the validation loss (x10) on both datasets in function of the cumulated length $L_c=N\cdot L$.}
\label{tab:lc_median}
\end{table*}

==> table_mean_snap.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{E14430}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{F98E52}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 3.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFBB9}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.44}} & \makebox[\linewidth]{{\cellcolor[HTML]{8EC2DC}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.60}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{E34933}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFF1AA}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.56}} & \makebox[\linewidth]{{\cellcolor[HTML]{F3FBD4}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.25}} & \makebox[\linewidth]{{\cellcolor[HTML]{3B56A5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.17}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.29}} & \makebox[\linewidth]{{\cellcolor[HTML]{F7814C}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 3.66}} & \makebox[\linewidth]{{\cellcolor[HTML]{97C9E0}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.64}} & \makebox[\linewidth]{{\cellcolor[HTML]{3A54A4}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.16}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FDB769}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.18}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED485}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.90}} & \makebox[\linewidth]{{\cellcolor[HTML]{78B0D3}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.50}} & \makebox[\linewidth]{{\cellcolor[HTML]{3F62AB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.20}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FEE090}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.80}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDE8E}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.81}} & \makebox[\linewidth]{{\cellcolor[HTML]{9BCCE2}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.66}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{D42D27}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED081}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.94}} & \makebox[\linewidth]{{\cellcolor[HTML]{97C9E0}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.64}} & \makebox[\linewidth]{{\cellcolor[HTML]{426CB0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.23}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{F57547}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 3.78}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED081}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.93}} & \makebox[\linewidth]{{\cellcolor[HTML]{78B0D3}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.50}} & \makebox[\linewidth]{{\cellcolor[HTML]{4D7FB9}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.30}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{FFF8B5}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.46}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.84}} & \makebox[\linewidth]{{\cellcolor[HTML]{6DA4CC}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.45}} & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.07}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FED889}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.87}} & \makebox[\linewidth]{{\cellcolor[HTML]{D1ECF4}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.95}} & \makebox[\linewidth]{{\cellcolor[HTML]{4A7AB7}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.28}} & \makebox[\linewidth]{{\cellcolor[HTML]{36479E}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.13}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FED687}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.88}} & \makebox[\linewidth]{{\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.72}} & \makebox[\linewidth]{{\cellcolor[HTML]{4F81BA}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.31}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{F7844E}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 3.64}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.85}} & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.69}} & \makebox[\linewidth]{{\cellcolor[HTML]{5385BD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.32}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{FED687}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.87}} & \makebox[\linewidth]{{\cellcolor[HTML]{D6EEF5}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.97}} & \makebox[\linewidth]{{\cellcolor[HTML]{4878B6}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.28}} & \makebox[\linewidth]{{\cellcolor[HTML]{3A54A4}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.16}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{FEE79B}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.69}} & \makebox[\linewidth]{{\cellcolor[HTML]{EAF7E6}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.14}} & \makebox[\linewidth]{{\cellcolor[HTML]{5183BB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.31}} & \makebox[\linewidth]{{\cellcolor[HTML]{4065AC}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.21}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FED081}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.94}} & \makebox[\linewidth]{{\cellcolor[HTML]{C5E6F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.88}} & \makebox[\linewidth]{{\cellcolor[HTML]{416AAF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{384CA0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.14}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FEE294}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.75}} & \makebox[\linewidth]{{\cellcolor[HTML]{D6EEF5}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.97}} & \makebox[\linewidth]{{\cellcolor[HTML]{4D7FB9}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.30}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_mean_snap.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Mean values of the validation loss (x10) on the snapshot dataset.}
\label{tab:loss_mean_snap}
\vspace{-0.5em}\end{table*}

==> table_mean_threshratio.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 7.49}} & \makebox[\linewidth]{{\cellcolor[HTML]{F57748}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.40}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDBF71}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.50}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFAB7}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.59}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{C01A27}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 6.89}} & \makebox[\linewidth]{{\cellcolor[HTML]{FBA35C}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.88}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE496}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.01}} & \makebox[\linewidth]{{\cellcolor[HTML]{C1E4EF}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.75}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{E54E35}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.97}} & \makebox[\linewidth]{{\cellcolor[HTML]{F67A49}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.37}} & \makebox[\linewidth]{{\cellcolor[HTML]{CBE9F2}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.84}} & \makebox[\linewidth]{{\cellcolor[HTML]{8ABEDA}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.36}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{E65036}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.93}} & \makebox[\linewidth]{{\cellcolor[HTML]{F57245}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.46}} & \makebox[\linewidth]{{\cellcolor[HTML]{EAF7E6}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.15}} & \makebox[\linewidth]{{\cellcolor[HTML]{3A51A2}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.75}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{ED5F3C}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.72}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED283}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{BBE1ED}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.71}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{EC5C3B}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.75}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDC576}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFF5AF}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.67}} & \makebox[\linewidth]{{\cellcolor[HTML]{E9F6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.14}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{FA9656}} \color[HTML]{000000} \raisebox{-1pt}{\small 5.01}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDE8E}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.10}} & \makebox[\linewidth]{{\cellcolor[HTML]{E5F5EF}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.08}} & \makebox[\linewidth]{{\cellcolor[HTML]{85BBD9}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.34}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{F8864F}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE699}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.95}} & \makebox[\linewidth]{{\cellcolor[HTML]{A6D5E7}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.54}} & \makebox[\linewidth]{{\cellcolor[HTML]{578ABF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.02}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FDB366}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.68}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE99D}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.91}} & \makebox[\linewidth]{{\cellcolor[HTML]{6DA4CC}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.17}} & \makebox[\linewidth]{{\cellcolor[HTML]{4F81BA}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.97}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FDC576}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{CDEAF3}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.86}} & \makebox[\linewidth]{{\cellcolor[HTML]{4471B2}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.89}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{FCAA5F}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.77}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE294}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.02}} & \makebox[\linewidth]{{\cellcolor[HTML]{FBFDC7}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.43}} & \makebox[\linewidth]{{\cellcolor[HTML]{BBE1ED}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.71}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{FDBF71}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.52}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEEDA4}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.82}} & \makebox[\linewidth]{{\cellcolor[HTML]{C3E5F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.77}} & \makebox[\linewidth]{{\cellcolor[HTML]{72ABD0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.21}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{FDC576}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.44}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEEA9F}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.88}} & \makebox[\linewidth]{{\cellcolor[HTML]{9BCCE2}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.48}} & \makebox[\linewidth]{{\cellcolor[HTML]{4B7DB8}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.95}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FDC374}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.46}} & \makebox[\linewidth]{{\cellcolor[HTML]{F3FBD4}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.32}} & \makebox[\linewidth]{{\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.20}} & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.64}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FDC778}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.40}} & \makebox[\linewidth]{{\cellcolor[HTML]{99CAE1}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.47}} & \makebox[\linewidth]{{\cellcolor[HTML]{E9F6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.15}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_mean_threshratio.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Mean values of the validation loss (x10) on the Threshold-Ratio dataset.}
\label{tab:loss_mean_threshratio}
\vspace{-0.5em}\end{table*}

==> table_time_mad_snap.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.23}} & \makebox[\linewidth]{{\cellcolor[HTML]{4A7AB7}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.11}} & \makebox[\linewidth]{{\cellcolor[HTML]{D8EFF6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.34}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFBB9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.59}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{74ADD1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.16}} & \makebox[\linewidth]{{\cellcolor[HTML]{8ABEDA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{E1F3F6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.37}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFBB9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.59}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.23}} & \makebox[\linewidth]{{\cellcolor[HTML]{B0DCEA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.25}} & \makebox[\linewidth]{{\cellcolor[HTML]{F7814C}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.70}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE79B}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.76}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FFF7B3}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.62}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDB769}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.49}} & \makebox[\linewidth]{{\cellcolor[HTML]{D62F27}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.95}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{E75337}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.34}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDB164}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.25}} & \makebox[\linewidth]{{\cellcolor[HTML]{F8864F}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.65}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{C1E4EF}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.29}} & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.24}} & \makebox[\linewidth]{{\cellcolor[HTML]{D8EFF6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.34}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{74ADD1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.16}} & \makebox[\linewidth]{{\cellcolor[HTML]{A6D5E7}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.23}} & \makebox[\linewidth]{{\cellcolor[HTML]{C9E8F2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.31}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFCBA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.58}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{C5E6F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.30}} & \makebox[\linewidth]{{\cellcolor[HTML]{FAFDC9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.51}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFF0A8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.69}} & \makebox[\linewidth]{{\cellcolor[HTML]{FCAA5F}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.30}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{F8FCCB}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.51}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEEFA6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.69}} & \makebox[\linewidth]{{\cellcolor[HTML]{F2FAD6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.47}} & \makebox[\linewidth]{{\cellcolor[HTML]{F99153}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.55}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FFF5AF}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.64}} & \makebox[\linewidth]{{\cellcolor[HTML]{FA9656}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.49}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFDBC}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.57}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.07}} & \makebox[\linewidth]{{\cellcolor[HTML]{AAD8E9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.24}} & \makebox[\linewidth]{{\cellcolor[HTML]{7DB4D5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.17}} & \makebox[\linewidth]{{\cellcolor[HTML]{AEDBEA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.25}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.23}} & \makebox[\linewidth]{{\cellcolor[HTML]{74ADD1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.16}} & \makebox[\linewidth]{{\cellcolor[HTML]{C5E6F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.30}} & \makebox[\linewidth]{{\cellcolor[HTML]{FBFDC7}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.52}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{72ABD0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.16}} & \makebox[\linewidth]{{\cellcolor[HTML]{BDE2EE}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.28}} & \makebox[\linewidth]{{\cellcolor[HTML]{D8EFF6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.35}} & \makebox[\linewidth]{{\cellcolor[HTML]{E9F6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.41}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{B6DFEC}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{F5FBD2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.48}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED485}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.94}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDBF71}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.12}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FEFFC0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.56}} & \makebox[\linewidth]{{\cellcolor[HTML]{FB9D59}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{EA5739}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.25}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_time_mad_snap.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Median Absolute Deviation (MAD) values of the training time (in hours) on the snapshot dataset.}
\label{tab:time_mad_snap}
\vspace{-0.5em}\end{table*}

==> table_time_mad_threshratio.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{659BC8}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.17}} & \makebox[\linewidth]{{\cellcolor[HTML]{94C7DF}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.23}} & \makebox[\linewidth]{{\cellcolor[HTML]{4676B5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.13}} & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.09}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{374A9F}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.10}} & \makebox[\linewidth]{{\cellcolor[HTML]{B9E0ED}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.30}} & \makebox[\linewidth]{{\cellcolor[HTML]{C3E5F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.33}} & \makebox[\linewidth]{{\cellcolor[HTML]{87BDD9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{FEFFC0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.59}} & \makebox[\linewidth]{{\cellcolor[HTML]{E4F4F1}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{C3E5F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.33}} & \makebox[\linewidth]{{\cellcolor[HTML]{EC5C3B}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.04}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FEE699}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.80}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDAD60}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.28}} & \makebox[\linewidth]{{\cellcolor[HTML]{FA9B58}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{AD0826}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 3.73}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FBFDC7}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.56}} & \makebox[\linewidth]{{\cellcolor[HTML]{CA2427}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 2.98}} & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.00}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{72ABD0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{78B0D3}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.09}} & \makebox[\linewidth]{{\cellcolor[HTML]{5385BD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.14}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{5A8EC1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.15}} & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{5588BE}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.15}} & \makebox[\linewidth]{{\cellcolor[HTML]{D8EFF6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.38}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.27}} & \makebox[\linewidth]{{\cellcolor[HTML]{F0F9DB}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.49}} & \makebox[\linewidth]{{\cellcolor[HTML]{E0F3F8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.40}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDC8C}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.90}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{8EC2DC}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{FAFDC9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDAF62}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{F88950}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 1.56}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FECE7F}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.99}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDBF71}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.12}} & \makebox[\linewidth]{{\cellcolor[HTML]{FB9D59}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.39}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{578ABF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.15}} & \makebox[\linewidth]{{\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.18}} & \makebox[\linewidth]{{\cellcolor[HTML]{69A0CA}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.17}} & \makebox[\linewidth]{{\cellcolor[HTML]{8ABEDA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{D1ECF4}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.37}} & \makebox[\linewidth]{{\cellcolor[HTML]{5385BD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.14}} & \makebox[\linewidth]{{\cellcolor[HTML]{3B56A5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.11}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE294}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.84}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{8ABEDA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{A3D3E6}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{4065AC}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.12}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFF5AF}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.67}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{ECF8E2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.47}} & \makebox[\linewidth]{{\cellcolor[HTML]{D1ECF4}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.36}} & \makebox[\linewidth]{{\cellcolor[HTML]{87BDD9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDAF62}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.26}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{ECF8E2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.47}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDAD60}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.28}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDC576}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.06}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_time_mad_threshratio.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Median Absolute Deviation (MAD) values of the training time (in hours) on the Threshold-Ratio dataset.}
\label{tab:time_mad_threshratio}
\vspace{-0.5em}\end{table*}

==> table_time_mean_snap.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{9DCEE3}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.79}} & \makebox[\linewidth]{{\cellcolor[HTML]{4676B5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.43}} & \makebox[\linewidth]{{\cellcolor[HTML]{9BCCE2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.78}} & \makebox[\linewidth]{{\cellcolor[HTML]{DEF2F7}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.21}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{8CC0DB}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.71}} & \makebox[\linewidth]{{\cellcolor[HTML]{B9E0ED}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.95}} & \makebox[\linewidth]{{\cellcolor[HTML]{D1ECF4}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.13}} & \makebox[\linewidth]{{\cellcolor[HTML]{FCA55D}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.72}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{99CAE1}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.77}} & \makebox[\linewidth]{{\cellcolor[HTML]{B2DDEB}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.91}} & \makebox[\linewidth]{{\cellcolor[HTML]{FB9D59}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.89}} & \makebox[\linewidth]{{\cellcolor[HTML]{FBA35C}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.80}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FFFAB7}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.87}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDBB6D}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.24}} & \makebox[\linewidth]{{\cellcolor[HTML]{BB1526}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 8.82}} & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 10.30}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{E34933}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 6.22}} & \makebox[\linewidth]{{\cellcolor[HTML]{F88950}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.35}} & \makebox[\linewidth]{{\cellcolor[HTML]{DA362A}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 6.90}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.59}} & \makebox[\linewidth]{{\cellcolor[HTML]{6297C6}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.53}} & \makebox[\linewidth]{{\cellcolor[HTML]{AEDBEA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.88}} & \makebox[\linewidth]{{\cellcolor[HTML]{AEDBEA}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.88}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{4676B5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.43}} & \makebox[\linewidth]{{\cellcolor[HTML]{5385BD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.47}} & \makebox[\linewidth]{{\cellcolor[HTML]{C5E6F0}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.03}} & \makebox[\linewidth]{{\cellcolor[HTML]{E7F6EB}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.35}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{AAD8E9}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.86}} & \makebox[\linewidth]{{\cellcolor[HTML]{9BCCE2}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.78}} & \makebox[\linewidth]{{\cellcolor[HTML]{ECF8E2}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{FCAA5F}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.61}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{FFF6B1}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.96}} & \makebox[\linewidth]{{\cellcolor[HTML]{F3FBD4}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.53}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEECA2}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.18}} & \makebox[\linewidth]{{\cellcolor[HTML]{E44C34}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 6.12}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FDFEC2}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.72}} & \makebox[\linewidth]{{\cellcolor[HTML]{F57547}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.82}} & \makebox[\linewidth]{{\cellcolor[HTML]{F88950}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.34}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.30}} & \makebox[\linewidth]{{\cellcolor[HTML]{76AFD2}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.62}} & \makebox[\linewidth]{{\cellcolor[HTML]{6BA2CB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.57}} & \makebox[\linewidth]{{\cellcolor[HTML]{E0F3F8}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.24}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{6297C6}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.53}} & \makebox[\linewidth]{{\cellcolor[HTML]{6DA4CC}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.58}} & \makebox[\linewidth]{{\cellcolor[HTML]{C1E4EF}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.01}} & \makebox[\linewidth]{{\cellcolor[HTML]{EAF7E6}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.38}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{83B9D8}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.67}} & \makebox[\linewidth]{{\cellcolor[HTML]{A1D1E5}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.81}} & \makebox[\linewidth]{{\cellcolor[HTML]{EBF7E4}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.39}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE496}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.39}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{B4DEEC}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.92}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFF5AF}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.97}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDAD60}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.60}} & \makebox[\linewidth]{{\cellcolor[HTML]{F57245}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.89}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FEECA2}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.19}} & \makebox[\linewidth]{{\cellcolor[HTML]{F88C51}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 4.26}} & \makebox[\linewidth]{{\cellcolor[HTML]{BE1827}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 8.53}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_time_mean_snap.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Mean values of the training time (in hours) on the snapshot dataset.}
\label{tab:time_mean_snap}
\vspace{-0.5em}\end{table*}

==> table_time_mean_threshratio.tex <==
\begin{table*}[p]
\centering
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}4096} & \makebox[0.8\linewidth][c]{\color{gray}8192} & \makebox[1.1\linewidth][c]{\color{gray}16384} & \makebox[1.4\linewidth][c]{\color{gray}32768} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{333D99}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.44}} & \makebox[\linewidth]{{\cellcolor[HTML]{4A7AB7}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.62}} & \makebox[\linewidth]{{\cellcolor[HTML]{69A0CA}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.77}} & \makebox[\linewidth]{{\cellcolor[HTML]{374A9F}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.47}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{4167AD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{9BCCE2}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.06}} & \makebox[\linewidth]{{\cellcolor[HTML]{97C9E0}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.04}} & \makebox[\linewidth]{{\cellcolor[HTML]{A6D5E7}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.14}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{CDEAF3}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.46}} & \makebox[\linewidth]{{\cellcolor[HTML]{9FD0E4}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.09}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFCBA}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.38}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDB567}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.32}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{DAF0F6}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.58}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEE79B}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.97}} & \makebox[\linewidth]{{\cellcolor[HTML]{FA9B58}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.94}} & \makebox[\linewidth]{{\cellcolor[HTML]{CC2627}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 9.49}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{F67F4B}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.74}} & \makebox[\linewidth]{{\cellcolor[HTML]{E54E35}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 7.42}} & \makebox[\linewidth]{{\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 12.39}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 1}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}8192} & \makebox[0.8\linewidth][c]{\color{gray}16384} & \makebox[1.1\linewidth][c]{\color{gray}32768} & \makebox[1.4\linewidth][c]{\color{gray}65536} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{3A51A2}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.50}} & \makebox[\linewidth]{{\cellcolor[HTML]{578ABF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.67}} & \makebox[\linewidth]{{\cellcolor[HTML]{394FA1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.49}} & \makebox[\linewidth]{{\cellcolor[HTML]{313695}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.43}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{5385BD}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.67}} & \makebox[\linewidth]{{\cellcolor[HTML]{3F62AB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{6BA2CB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.78}} & \makebox[\linewidth]{{\cellcolor[HTML]{C9E8F2}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.42}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{5A8EC1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.70}} & \makebox[\linewidth]{{\cellcolor[HTML]{92C5DE}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.01}} & \makebox[\linewidth]{{\cellcolor[HTML]{DCF1F7}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.59}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEEA9F}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.88}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{D8EFF6}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.55}} & \makebox[\linewidth]{{\cellcolor[HTML]{AEDBEA}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.20}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDC778}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.79}} & \makebox[\linewidth]{{\cellcolor[HTML]{FDB164}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.38}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{FFFDBC}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.33}} & \makebox[\linewidth]{{\cellcolor[HTML]{FECE7F}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.64}} & \makebox[\linewidth]{{\cellcolor[HTML]{F98E52}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 5.33}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 2}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\textwidth}
\centering
\small \begin{tabularx}{\linewidth}{{lXXXX}}
\toprule
\makebox[25pt][r]{$L$} & \makebox[0.5\linewidth][c]{4096} & \makebox[0.8\linewidth][c]{8192} & \makebox[1.1\linewidth][c]{16384} & \makebox[1.4\linewidth][c]{32768} \\
$B$ \textbackslash~ {\color{gray} $L_c$} & \makebox[0.5\linewidth][c]{\color{gray}12288} & \makebox[0.8\linewidth][c]{\color{gray}24576} & \makebox[1.1\linewidth][c]{\color{gray}49152} & \makebox[1.4\linewidth][c]{\color{gray}98304} \\
\midrule
8 & \makebox[\linewidth]{{\cellcolor[HTML]{5A8EC1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.70}} & \makebox[\linewidth]{{\cellcolor[HTML]{6095C4}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.73}} & \makebox[\linewidth]{{\cellcolor[HTML]{5A8EC1}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.70}} & \makebox[\linewidth]{{\cellcolor[HTML]{4676B5}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.61}} \\
16 & \makebox[\linewidth]{{\cellcolor[HTML]{72ABD0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.83}} & \makebox[\linewidth]{{\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.81}} & \makebox[\linewidth]{{\cellcolor[HTML]{3E60AA}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.54}} & \makebox[\linewidth]{{\cellcolor[HTML]{BFE3EF}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.33}} \\
32 & \makebox[\linewidth]{{\cellcolor[HTML]{588CC0}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.69}} & \makebox[\linewidth]{{\cellcolor[HTML]{6BA2CB}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.79}} & \makebox[\linewidth]{{\cellcolor[HTML]{70A9CF}} \color[HTML]{F1F1F1} \raisebox{-1pt}{\small 0.82}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEEFA6}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.73}} \\
64 & \makebox[\linewidth]{{\cellcolor[HTML]{7AB2D4}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.87}} & \makebox[\linewidth]{{\cellcolor[HTML]{81B7D7}} \color[HTML]{000000} \raisebox{-1pt}{\small 0.91}} & \makebox[\linewidth]{{\cellcolor[HTML]{FFFEBE}} \color[HTML]{000000} \raisebox{-1pt}{\small 2.30}} & \makebox[\linewidth]{{\cellcolor[HTML]{FEDA8A}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.35}} \\
128 & \makebox[\linewidth]{{\cellcolor[HTML]{A8D6E8}} \color[HTML]{000000} \raisebox{-1pt}{\small 1.15}} & \makebox[\linewidth]{{\cellcolor[HTML]{FED889}} \color[HTML]{000000} \raisebox{-1pt}{\small 3.38}} & \makebox[\linewidth]{{\cellcolor[HTML]{FB9D59}} \color[HTML]{000000} \raisebox{-1pt}{\small 4.91}} &  \\
\bottomrule
\end{tabularx}
\captionsetup{skip=2pt}
\caption{N = 3}
\end{subtable}
\hfill
\begin{subtable}[h]{0.05\linewidth}
\centering
\includegraphics[height=70pt]{cbar_time_mean_threshratio.pdf}
\vfill \vspace{-0.5em}
\end{subtable}
\hfill
\caption{Mean values of the training time (in hours) on the Threshold-Ratio dataset.}
\label{tab:time_mean_threshratio}
\vspace{-0.5em}\end{table*}
